Queue or lounge: strategic design for strategic customer

Considering an M/M/1 queue with an additional lounge facility (LF), the quest of this paper is to understand the instances when LF is an attractive option, from customer perspective as well as from system perspective: will the customers choose to join the queue or prefer to detour briefly to lounge? In reality, customers do not perform complex computations for such tasks, but instead choose based on some heuristics. We further assume that the customers pessimistically anticipate the future congestion while making the choice. Our analysis reveals that the customers use the LF only when the queue is too crowded, and the lounge is relatively empty; however, strikingly, the customer choice is more inclined towards rejection for the LF in systems with higher traffic (load). We also explore an optimization problem where the system determines whether to implement an LF and what capacity it should have, while accounting for customers' behavioral responses. Under low load conditions, the system benefits from designing a high-capacity lounge, and the customers also prefer to use the LF actively. Surprisingly, neither the system prefers big LF, nor the customers prefer to use the LF profusely at high load conditions; optimal for either is to use the LF sparingly. Thus, importantly, the strategic system and the bounded-rational customers are not in a tug-of-war situation.

==> Proof.tex <==

\newcommand{\bpi}{{\bm \pi}}
\newcommand{\X}{{\cal X}}
\newcommand{\barnu}{ {\bar \nu}}

The idea is to write the stationary distribution as a unique zero of an appropriate function, given its existence (proved in s..).
And then discuss the continuity of this minimizer using maximum theorem. 
There are two steps: i) to construct an appropriate function,  an appropriate domain and topology ii) to prove required continuity compactness arguments. 

{\bf Step  1} The variable is $\bpi = \{\pi_{q,l}  \}$ and consider the function following real-valued function of $\bpi$
\begin{eqnarray}
    \Gamma (\bpi; \nu ) &:= & \sum_{ql} \rho^{q+l} f_{ql} (\bpi; \nu) \mbox{ with }  \\
    f_{ql} (\bpi; \nu)  &:= & | b_{ql} (\bpi; \nu) - \pi_{ql} |
 \end{eqnarray}
 where $b_{ql} (\bpi)$ represents the RHS of the balance equation as given in \eqref{eq_q=00}-\eqref{eq_lBq>A+1} after replacing $\beta = \eta \nu$, where $\eta > 0$ is fixed constant and treating $\mu, \lambda, \alpha$ as fixed constants.
 For the domain  the following set is appropriate:
 \begin{eqnarray}
 \D :=  \left \{ \bpi : \pi_{ql } \ge 0 \mbox{ and }  \sum_{ql} \pi_{ql} = 1 \right \}.    
 \end{eqnarray}

 Let $\X := [[0,1]\times[0,1] ]^\infty$ be a product space equipped with product topology   (which ensures component-wise continuity or continuity of projections), basically 
 $$
 \bpi^n \to \bpi  \mbox{ if distance, }  d_T (\bpi^n, \bpi) :=  \sum_{ql} 2^{-(q+l)} \frac{ |\pi^n_{ql} - \pi_{ql}| }{1 +|\pi^n_{ql} - \pi_{ql}| } \to 0
 $$
 which is equivalent to 
 $$
 \pi^n_{ql} \to \pi_{ql} \mbox{ for every } q,l. 
 $$
 By Tychonoff's theorem under the product topology given by  metric $d_T$, $\X$ is compact.  Since clearly $\D \subset \X$, which is closed it is also compact. 
 Thus, 
 $$
 \Gamma : \D \times  [0, \barnu] \to \mathcal{R}
 $$
 for some $\barnu < \infty $ and where $D$ is equipped with product topology.

 {\bf Step 2:}  We will now show the joint continuity of $\Gamma$, sufficient to show sequential continuity. Now consider a sequence $(\bpi^n, \nu^n)$ and a tuple $(\bpi, \nu)$ such that $d_T(\bpi^n, \bpi) \to 0$ and $\nu^n \to \nu$, then we need to show that, 
 \begin{eqnarray*}
     \Gamma(\bpi^n, \nu^n) \to \Gamma ((\bpi, \nu) \mbox{ as } n\to \infty. 
 \end{eqnarray*}
 {\bf Step 2.a:} Prove it for $\nu > 0$ using bounded convergence theorem, and component-wise convergence, basically show  $b_
 {ql}(\bpi^n) \to b_{ql} (\bpi)$ for every $ql$ and then BCT. 

 {\bf Step 2.b:} For $\nu = 0$, we need to truncate the tail and then ...


  \subsection{Connection between the limiting system and JDS system}
{\color{red}Join the Queue Later  (JQL) or Jump Directly to the Server  (JDS)

At limit we have another Lounge facility system, where the customers are encouraged to move to the Lounge and are guaranteed to be informed of the instance the server becomes empty (so as to directly move for their service)  when the server  The tokens for service in Lounge queue are also FCFS based. }


% In the heavy-traffic regime, the JQL (Join-the-Queue-or-Lounge) system exhibits behavior akin to a system where customers are encouraged to enter a Lounge area.
% In this configuration, customers in the Lounge are guaranteed to be informed the moment the server becomes idle, allowing them to directly receive service without rejoining the main queue. Service tokens in the Lounge are allocated on a first-come, first-served (FCFS) basis, effectively forming a virtual queue that ensures fairness among Lounge participants. We refer to this mechanism as `join directly to the server'.

% In this model, once a customer decides to enter the Lounge, they are assured of receiving service immediately upon server availability and subsequently exit the system.

The `FDS' policy described above proposes a slightly modified system where, the customers are routed to the lounge if the  waiting cost for expected delay in the main queue exceeds the cost of total expected delay generated by the joint occupancy of both the main queue and the lounge. This is because, the customers waiting in lounge are allowed to enter server once the server is empty and all the customers ahead in lounge exists the system. This leads to the following decision criterion for lounge entry:
\begin{align}
    \frac{\alpha Q}{\mu} &> (Q+L) \cdot \text{E(busy period)} \cdot \beta, \nonumber \\
  \implies   Q &>  \frac{\mu \beta L}{\mu(\alpha - \beta) - \lambda \alpha}.
\end{align}
This condition yields a dynamic threshold for queue length that  explicitly incorporates current Lounge occupancy. Interestingly The model is valid and insightful under high-traffic conditions as well.

     
 \section{Lounge problem}
 {\color{red}We now discuss this problem from the system perspective. Basically the aim in this section is to understand what is beneficial for the system. Even more fundamental question to be answered is, if the systems finds it beneficial to design a lounge. More so at heavy traffic condition  (where there is an expectation that lounge design can ease \cite{Juneja}).


The design of lounge can be represented by choosing  parameter $\eta$ optimally.  -- optimality -- budget . and congestion cost 

This problem can be viewed as two level optimization problem or stakel berge game problem, with an exception that we just have a response function of the customers at the lower level as given by Theorem 1.. Let $M(\eta)$ represent the monetary budget associated with design of a lounge with comfortness factor $\eta$.  Let $G(\eta)$ represent the total congestion of the system (including that in Lounge) for given $\eta$ -- observe here that, given $\eta$ there is a response by customer given by $A(\eta) = \eta \nicefrac{\mu}{\alpha}$ and $B = \nicefrac{\mu-\lambda}{\nu} - A(\eta) $ (Thm ..). which drives the system Markov chain $(Q_t, L_t)$ and the resultant stationary distribution  determines the congestion cost. 

In other words one can view $\bpi = \{\pi_{ql}\}_{q,l} =:\bpi(A(\eta)) $ as the response of the customers for the choice $\eta$ of the system and then  thus $G(\eta) = G(\bpi (A(\eta) ) $ represents the congestion cost:
\begin{eqnarray*}
    G(\eta) = \sum_{q,l} \pi_{ql} (A(\eta) ) g(q,l)
\end{eqnarray*}
where $g(q,l)$ represents the congestion cost at queue lounge occupancy levels $(q,l).$}




